FALKON: An Optimal Large Scale Kernel Method

Kernel methods provide a principled way to perform non linear, nonparametric learning. They rely on solid functional analytic foundations and enjoy optimal statistical properties. However, at least in their basic form, they have limited applicability in large scale scenarios because of stringent computational requirements in terms of time and especially memory. In this paper, we take a substantial step in scaling up kernel methods, proposing FALKON, a novel algorithm that allows to efficiently process millions of points. FALKON is derived combining several algorithmic principles, namely stochastic subsampling, iterative solvers and preconditioning. Our theoretical analysis shows that optimal statistical accuracy is achieved requiring essentially $O(n)$ memory and $O(n\sqrt{n})$ time. An extensive experimental analysis on large scale datasets shows that, even with a single machine, FALKON outperforms previous state of the art solutions, which exploit parallel/distributed architectures.

==> Experiments/EXP_long.tex <==

\section{Experiments}

In this section we present Falcon's performance on a range of largre scale datasets.
We measure the results with the MSE, RMSE or Relative error for regularization problems,
and with the c-error or AUC for the classification problems.
Falcon was coded in MATLAB and run on a single machine equipped with two Intel Xeon
E$5$-$2630$ v$3$ ($2.4$ GHz, $8$ cores each), one NVIDIA
Tesla K$40$c and $128$ GB of RAM. For HIGGS, YELP and SUSY datsets where there is not
a fixed test set, we split the data in 80\% for training and 20\% for testing.
For all datasets apart from YELP we normalize the features by their z-score.

{\bf MILLIONSONGS} The first experiment tests Falcon on MillionSongs \cite{BertinMahieux2011TheMS},
a dataset made of \num[group-separator={,}]{463715} training and
\num[group-separator={,}]{51630} testing points of dimensionnality $90$.
Each example represent a song and the learning goal is to predict the year in which it
was released.
We use the same preprocessing, kernel and $\sigma$ as \cite{conf/colt/ZhangDW13}.
In Table~\ref{Millionsongs_table} we observe our result when we choose \num[group-separator={,}]{10000} Nystrom centers
and $lambda = 10^{-6}$. With this setting Falcon is abel to reach the competitors in less than a minute.
Increasing the Nystrom centers to \num[group-separator={,}]{50000} it gets to a MSE of $79.20$ and a Relative error of $4.49\times10^{-3}$ in $630$ \textit{sec}.

\begin{table}[h]
  \label{Millionsongs_table}
  \centering

\end{table}


{\bf HIGGS}~We evaluate a classification task on the HIGGS Dataset\footnote{\url{https://archive.ics.uci.edu/ml/datasets/HIGGS}}
where the goal is to distinguish between a signal process which produces Higgs
bosons and a background process which does not.
%
The dataset consists of $1.1\times 10^6$ points of dimensionality $28$.
%
Results from Table~\ref{HIGGS_table} are obtained using a Gaussian Kernel of width $\sigma = 5$, $\lambda = 1\times10^{-8}$ and
$1\times10^5$ Nystrom centers.
Falcon is reach the accuracy of NN e BDT with the DNN still a bit ahead.
Note that if we enrich our model a bit using a Gaussian kernel with diagona matrix width learned with cross validation, Falcon reaches an AUC of $0.830$.

The time referes to the same experiment performed by \cite{Alves2016StackingML} on a single machine.
\begin{table}[h]
  \caption{HIGGS Dataset}
  \label{HIGGS_table}
  \centering
    \begin{tabular}{lccc}
      \toprule
       MILLIONSONGS    & MSE   &Relative Error            & Time(\textit{sec})\\
      \midrule
      Falcon                      & \textbf{80.30}  &$\mathbf{4.51\times10^{-3}}$    & \textbf{55}  \\
      Prec. KRR\cite{avron2016faster}                 &-               &$4.58\times10^{-3}$    &289 \\
      Hierarchical \cite{Chen2016HierarchicallyCK}                 &-               &$4.56\times10^{-3}$    &293 \\
      D\&C \cite{conf/colt/ZhangDW13}            & 80.35    &-             & 737 \\
      Rand. Feat. \cite{conf/colt/ZhangDW13}     & 80.93    &-            & 772 \\
      Nystrom \cite{conf/colt/ZhangDW13}             & 80.38    &-            & 876 \\
      ADMM\cite{avron2016faster}                 &-               &$5.01\times10^{-3}$    &958 \\
      \bottomrule
    \end{tabular}
      \begin{tabular}{lcc}
        \toprule
         HIGGS                           & AUC   & Time (\textit{hours})   \\
        \midrule
        Falcon                      & 0.818 & \textbf{3} \\
        BDT \cite{baldi2014searching}                 & 0.810 & - \\
        NN \cite{baldi2014searching}                  & 0.816 & - \\
        DNN \cite{baldi2014searching}                 & 0.885 & $78^*$ \\
        \bottomrule
      \end{tabular}

\end{table}

{\bf TIMIT}~The TIMIT dataset allow us to test Falcon on a multiclass classification task.
We used the same preprocessed dataset of [Mikhal] consisting of \num[group-separator={,}]{1124823}
training points and \num[group-separator={,}]{57242} test points of dimentionality $440$.
In this experiment (Table~\ref{TIMIT_table}) Falcon exploit a Gaussian Kernel of width $\sigma = 15$,
$\lambda = 10^{-9}$ and $10^5$ Nystrom centers.
% The results in Table~\ref{TIMIT_table}, shows that Falcon outperform most of the competitors
% (including a DNN and full KRR) in a small amount of time and only one machine. (IBM?)
% Notice that in respect to most competitors we train only on half the number of points. (WHY)
% **Our dataset adopts 10ms frames and drops the glottal stop \'q\' related labels,
% thus we ignore the relevant frames in core test set (1.2\% of total test set).
% Note that in the worst case, if we mislabel all these frames, the corresponding
% frame-level classification error will drop from 32.6\% to 33.39\%.**

\begin{table}[h]
  \caption{TIMIT Dataset}
  \label{TIMIT_table}
  \centering

  \begin{tabular}{lcccccc}
    \toprule
    TIMIT                         & Class error   & Time (\textit{hours})   \\
    \midrule
    Falcon                      & 32.31\% & \textbf{1.5} \\
    BCD Rand. Feat. \cite{tu2016large}   & 34.02\% & 1.7 \\
    BCD Nystrom \cite{tu2016large}           & 33.73\% & 1.7 \\
    EigenPro \cite{ma2017diving}            & 32.60\% & 3.9 \\
    KRR \cite{tu2016large}                   & 33.51\% & 8.3 \\
    Ensemble \cite{Huang2014KernelMM}          & 33.50\% & -   \\
    ????Kernels \cite{May2017KernelAM}    & 30.85\% & -   \\
    DNN \cite{May2017KernelAM}                   & 32.40\% & -   \\
    \bottomrule
  \end{tabular}
\end{table}

\begin{table}[h]
  \caption{YELP Dataset}
  \label{YELP_table}
  \centering
          \begin{tabular}{lcc}
            \toprule
             YELP                                       & RMSE              & Time (\textit{mins}) \\
            \midrule
            Falcon (M = 50K)                        & \textbf{0.833}    & $\textbf{20}$ \\
            BCD Hashing \cite{tu2016large}                       & 0.949             & $42^*$ \\
            BCD Nystrom \cite{tu2016large}                       & 0.861             & $60^*$ \\
            KRR  \cite{tu2016large}           & 0.854             & $500^*$ \\
            \bottomrule
          \end{tabular}
\end{table}

Experiments are performed on Amazon EC2 with a cluster of 128 r3.2xlarge machines, each of which has 4 physical cores and 62 GB of RAM.

{\bf YELP}~~In the end we compare ourself with the dataset YELP used by \cite{tu2016large},
made of $1.5 \times 10^6$ reviews. The goal is to predict a rating from one to five stars from the text of a review.
As preprocessing we extract the 3-grams from the plain text using the same pipeline described by \cite{tu2016large},
then we map them in a sparse vector of dimension $6.52 \times 10^7$ which record if the 3-gram is present or not in the example.
For the results presented in Table~\ref{YELP_table} Falcon uses a linear kernel with $5\times10^4$ Nystorm centers.
Increasing the number of centers to $10^5$ it reach a RMSE of $0.8280$ in $50$ minutes.

{\bf SUSY}~~For this dataset\footnote{\url{https://archive.ics.uci.edu/ml/datasets/SUSY}}, consisting of $5\times10^6$ examples of dimension $18$,
the goal is to distinguish between a process where SUSY particles are produced and one where they are not.
Results for Falcon with a Gaussina kernel of width $\sigma = 5$, $\lambda = 10^{-6}$ and $10^4$ Nystrom centers are shown
in Table~\ref{SUSY_table}.

\begin{table}[h]
  \caption{SUSY Dataset}
  \label{SUSY_table}
  \centering

  \begin{tabular}{lccc}
    \toprule
    SUSY                           & Class error    & AUC    & Time (\textit{min})   \\
    \midrule
    Falcon                          & \textbf{19.4\%}  &0.877   & \textbf{4} \\
    EigenPro \cite{ma2017diving}    & 19.8\%         &-       & 6 \\
    Hierarchical \cite{Chen2016HierarchicallyCK}                   & 20.1\%         &-       & 40 \\
    BDT \cite{baldi2014searching}                     &-              & 0.863     &- \\
    NN \cite{baldi2014searching}                   &-                 & 0.875    & -\\
    DNN \cite{baldi2014searching}                  &-                  &\textbf{0.879}     & 4680  \\
    \bottomrule
  \end{tabular}
\end{table}


==> Experiments/EXP_shortTable1.tex <==

\section{Experiments}

In this section we present Falcon's performance on a range of largre scale datasets.
We measure the results with the MSE, RMSE or Relative error for regularization problems,
and with the c-error or AUC for the classification problems.
Falcon was coded in MATLAB and run on a single machine equipped with two Intel Xeon
E$5$-$2630$ v$3$, one NVIDIA
Tesla K$40$c and $128$ GB of RAM. For datasets which have not a fixed test set,
we take apart 20\% of the data for testing.
For all datasets apart from YELP we normalize the features by their z-score.
We observe from the following results that FALCON is able to perform as well as state of
the art competitors if not better in a small fraction of their time.
From now on we denote with $n$ the cardinality of the dataset, $d$ the dimensionality.

{\bf MILLIONSONGS \cite{BertinMahieux2011TheMS}} ($n=\num[group-separator={,}]{463715}$, $d=90$, regression).
%
We use the same preprocessing, kernel and $\sigma$ as \cite{conf/colt/ZhangDW13}.
In Table~\ref{MS_table} we observe our result when we choose \num[group-separator={,}]{10000} Nystrom centers
and $lambda = 10^{-6}$.
Increasing the centers to \num[group-separator={,}]{50000} we get a MSE of $79.20$ and a Relative error of $4.49\times10^{-3}$ in $630$ \textit{sec}.

\begin{table}[h]
  \caption{MILLIONSONGS and SUSY Datasets. $\dagger = $ time obtained by \cite{Alves2016StackingML} working on a single machine.}
  \label{MS_table}
  \centering
    \begin{tabular}{lccc}
      \toprule
      %& \multicolumn{3}{c}{MILLIONSONGS Dataset} \\
      %\cmidrule{2-4}
      \textbf{MILLIONSONGS}
           & MSE   &Relative Error            & Time(\textit{sec})\\
      \midrule
      Falcon                      & \textbf{80.30}  &$\mathbf{4.51\times10^{-3}}$    & \textbf{55}  \\
      Prec. KRR\cite{avron2016faster}                 &-               &$4.58\times10^{-3}$    &289 \\
      Hierarchical \cite{Chen2016HierarchicallyCK}                 &-               &$4.56\times10^{-3}$    &293 \\
      D\&C \cite{conf/colt/ZhangDW13}            & 80.35    &-             & 737 \\
      Rand. Feat. \cite{conf/colt/ZhangDW13}     & 80.93    &-            & 772 \\
      Nystrom \cite{conf/colt/ZhangDW13}             & 80.38    &-            & 876 \\
      ADMM\cite{avron2016faster}                 &-               &$5.01\times10^{-3}$    &958 \\
      \bottomrule
      \toprule
    % \midrule
    %   & \multicolumn{3}{c}{SUSY Dataset} \\
    %   \cmidrule{2-4}
    \textbf{SUSY}
                                 & Class error    & AUC    & Time (\textit{min})   \\
      \midrule
      Falcon                          & \textbf{19.4\%}  &0.877   & \textbf{4} \\
      EigenPro \cite{ma2017diving}    & 19.8\%         &-       & 6 \\
      Hierarchical \cite{Chen2016HierarchicallyCK}                   & 20.1\%         &-       & 40 \\
      BDT \cite{baldi2014searching}                     &-              & 0.863     &- \\
      NN \cite{baldi2014searching}                   &-                 & 0.875    & -\\
      DNN \cite{baldi2014searching}                  &-                  &\textbf{0.879}     & $4680^\dagger$  \\
      \bottomrule
    \end{tabular}
\end{table}

{\bf TIMIT}~($n = \num[group-separator={,}]{1124823}$, $d = 440$, multiclass classification).
%
In this experiment we used the same preprocessed dataset of [Mikhal].
In the results of Table~\ref{YHT_table} Falcon exploits a Gaussian Kernel of width $\sigma = 15$,
$\lambda = 10^{-9}$ and $10^5$ Nystrom centers.
% The results in Table~\ref{TIMIT_table}, shows that Falcon outperform most of the competitors
% (including a DNN and full KRR) in a small amount of time and only one machine. (IBM?)
% Notice that in respect to most competitors we train only on half the number of points. (WHY)
% **Our dataset adopts 10ms frames and drops the glottal stop \'q\' related labels,
% thus we ignore the relevant frames in core test set (1.2\% of total test set).
% Note that in the worst case, if we mislabel all these frames, the corresponding
% frame-level classification error will drop from 32.6\% to 33.39\%.**

% \begin{table}[h]
%   \caption{TIMIT Dataset. $\ddagger = $ time obtained on a cluster of 128 Amazon r3.2xlarge machines.}
%   \label{TIMIT_table}
%   \centering
%
%   \begin{tabular}{lcccccc}
%     \toprule
%     TIMIT                         & Class error   & Time (\textit{hours})   \\
%     \midrule
%     Falcon                      & 32.3\% & \textbf{1.5} \\
%     BCD Rand. Feat. \cite{tu2016large}   & 34.0\% & $1.7^\ddagger$ \\
%     BCD Nystrom \cite{tu2016large}           & 33.7\% & $1.7^\ddagger$ \\
%     EigenPro \cite{ma2017diving}            & 32.6\% & 3.9 \\
%     KRR \cite{tu2016large}                   & 33.5\% & $8.3^\ddagger$ \\
%     DNN \cite{May2017KernelAM}                   & 32.4\% & -   \\
%     ????Kernels \cite{May2017KernelAM}    & \textbf{30.9\%} & -   \\
%     Ensemble \cite{Huang2014KernelMM}          & 33.5\% & -   \\
%     \bottomrule
%   \end{tabular}
% \end{table}



{\bf SUSY}~($n = 5\times10^6$, $d = 18$, binary classification).
%
Results for Falcon with a Gaussina kernel of width $\sigma = 5$, $\lambda = 10^{-6}$ and $10^4$ Nystrom centers are shown
in Table~\ref{MS_table}.

% \begin{table}[h]
%     \caption{SUSY Dataset. $\dagger = $ time obtained by \cite{Alves2016StackingML} working on a single machine.}
%     \label{SUSY_table}
%     \centering
%
%     \begin{tabular}{lccc}
%         \toprule
%         SUSY                           & Class error    & AUC    & Time (\textit{min})   \\
%         \midrule
%         Falcon                          & \textbf{19.4\%}  &0.877   & \textbf{4} \\
%         EigenPro \cite{ma2017diving}    & 19.8\%         &-       & 6 \\
%         Hierarchical \cite{Chen2016HierarchicallyCK}                   & 20.1\%         &-       & 40 \\
%         BDT \cite{baldi2014searching}                     &-              & 0.863     &- \\
%         NN \cite{baldi2014searching}                   &-                 & 0.875    & -\\
%         DNN \cite{baldi2014searching}                  &-                  &\textbf{0.879}     & $4680^\dagger$  \\
%         \bottomrule
%     \end{tabular}
% \end{table}

\begin{table}[h]
    \caption{YELP, HIGGS and TIMIT Datasets. $\dagger = $ time obtained by \cite{Alves2016StackingML} working on a single machine. $\ddagger = $ time obtained on a cluster of 128 Amazon r3.2xlarge machines.}
    \label{YHT_table}
    \begin{subtable}[]{0.3\linewidth}
        \centering
    \begin{tabular}{lcc}
        \toprule
        % & \multicolumn{2}{c}{YELP Dataset} \\
        % \cmidrule{2-3}
        \textbf{YELP}
                                               & RMSE              & Time (\textit{mins}) \\
        \midrule
        Falcon                      & \textbf{0.833}    & $\textbf{20}$ \\
        BCD Hashing \cite{tu2016large}                       & 0.949             & $42^\ddagger$ \\
        BCD Nystrom \cite{tu2016large}                       & 0.861             & $60^\ddagger$ \\
        KRR  \cite{tu2016large}           & 0.854             & $500^\ddagger$ \\
        \bottomrule
        \toprule
        %  \midrule
         % & \multicolumn{2}{c}{HIGGS Dataset} \\
         % \cmidrule{2-3}
         \textbf{HIGGS}
                                    & AUC   & Time (\textit{hours})   \\
         \midrule
         Falcon                      & 0.818 & \textbf{3} \\
         BDT \cite{baldi2014searching}                 & 0.810 & - \\
         NN \cite{baldi2014searching}                  & 0.816 & - \\
         DNN \cite{baldi2014searching}                 & \textbf{0.885} & $78^\dagger$ \\
        \bottomrule
    \end{tabular}
\end{subtable}
\hspace{2.2cm}
\begin{subtable}[]{0.3\linewidth}
        \centering
    \begin{tabular}{lcc}
      \toprule
    %   & \multicolumn{2}{c}{TIMIT Dataset} \\
    %   \cmidrule{2-3}
    \textbf{TIMIT}
                               & Class error   & Time (\textit{hours})   \\
      \midrule
      Falcon                      & 32.3\% & \textbf{1.5} \\
      BCD Rand. Feat. \cite{tu2016large}   & 34.0\% & $1.7^\ddagger$ \\
      BCD Nystrom \cite{tu2016large}           & 33.7\% & $1.7^\ddagger$ \\
      EigenPro \cite{ma2017diving}            & 32.6\% & 3.9 \\
      KRR \cite{tu2016large}                   & 33.5\% & $8.3^\ddagger$ \\
      DNN \cite{May2017KernelAM}                   & 32.4\% & -   \\
      ????Kernels \cite{May2017KernelAM}    & \textbf{30.9\%} & -   \\
      Ensemble \cite{Huang2014KernelMM}          & 33.5\% & -   \\
      \bottomrule
    \end{tabular}
    \end{subtable}
\end{table}

{\bf YELP}~~($n = 1.5 \times 10^6$, $d = 6.52 \times 10^7$, regression).
%
We test Falcon on the same dataset used by \cite{tu2016large},
For preprocessing we extract the 3-grams from the plain text with the same pipeline as \cite{tu2016large},
then we map them in a sparse vector which records if the 3-gram is present or not in the example.
For the results presented in Table~\ref{YHT_table} Falcon uses a linear kernel with $5\times10^4$ Nystorm centers.
Increasing the number of centers to $10^5$ we get a RMSE of $0.8280$ in $50$ minutes.

% \begin{table}[h]
%     \caption{YELP Dataset. $\ddagger = $ time obtained on a cluster of 128 Amazon r3.2xlarge machines.}
%     \label{YELP_table}
%     \begin{subtable}[t]{.45\linewidth}
%     \centering
%     \begin{tabular}{lcc}
%         \toprule
%         YELP                                       & RMSE              & Time (\textit{mins}) \\
%         \midrule
%         Falcon                      & \textbf{0.833}    & $\textbf{20}$ \\
%         BCD Hashing \cite{tu2016large}                       & 0.949             & $42^\ddagger$ \\
%         BCD Nystrom \cite{tu2016large}                       & 0.861             & $60^\ddagger$ \\
%         KRR  \cite{tu2016large}           & 0.854             & $500^\ddagger$ \\
%         \bottomrule
%     \end{tabular}
% \end{subtable}\hfill
%     \begin{subtable}[t]{.45\linewidth}
%         \begin{tabular}{lcc}
%         \toprule
%         HIGGS                           & AUC   & Time (\textit{hours})   \\
%         \midrule
%         Falcon                      & 0.818 & \textbf{3} \\
%         BDT \cite{baldi2014searching}                 & 0.810 & - \\
%         NN \cite{baldi2014searching}                  & 0.816 & - \\
%         DNN \cite{baldi2014searching}                 & \textbf{0.885} & $78^\dagger$ \\
%         \bottomrule
%         \end{tabular}
%     \end{subtable}
% \end{table}

{\bf HIGGS}~($n = 1.1\times 10^6$, $d = 28$, binary classification).
%
Results from Table~\ref{YHT_table} are obtained using a Gaussian Kernel of width $\sigma = 5$, $\lambda = 1\times10^{-8}$ and
$1\times10^5$ Nystrom centers.
If we enrich our model a bit using a Gaussian kernel with diagona matrix width learned with cross validation,
Falcon reaches an AUC of $0.830$.


% \begin{table}[h]
%     \caption{HIGGS Dataset. $\dagger = $ time obtained by \cite{Alves2016StackingML} working on a single machine.}
%     \label{HIGGS_table}
%     \centering
%     \begin{tabular}{lcc}
%         \toprule
%         HIGGS                         & AUC   & Time (\textit{hours})   \\
%         \midrule
%         Falcon                      & 0.818 & \textbf{3} \\
%         BDT \cite{baldi2014searching}                 & 0.810 & - \\
%         NN \cite{baldi2014searching}                  & 0.816 & - \\
%         DNN \cite{baldi2014searching}                 & \textbf{0.885} & $78^\dagger$ \\
%         \bottomrule
%         \toprule
%         YELP                                       & RMSE              & Time (\textit{mins}) \\
%         \midrule
%         Falcon                      & \textbf{0.833}    & $\textbf{20}$ \\
%         BCD Hashing \cite{tu2016large}                       & 0.949             & $42^\ddagger$ \\
%         BCD Nystrom \cite{tu2016large}                       & 0.861             & $60^\ddagger$ \\
%         KRR  \cite{tu2016large}           & 0.854             & $500^\ddagger$ \\
%         \bottomrule
%     \end{tabular}
% \end{table}


==> Experiments/EXP_shortTable2.tex <==

\section{Experiments}

In this section we present Falcon's performance on a range of largre scale datasets.
We measure the results with the MSE, RMSE or Relative error for regularization problems,
and with the c-error or AUC for the classification problems.
Falcon was coded in MATLAB and run on a single machine equipped with two Intel Xeon
E$5$-$2630$ v$3$, one NVIDIA
Tesla K$40$c and $128$ GB of RAM. For datasets which have not a fixed test set,
we take apart 20\% of the data for testing.
For all datasets apart from YELP we normalize the features by their z-score.
We observe from the following results that FALCON is able to perform as well as state of
the art competitors if not better in a small fraction of their time.
From now on we denote with $n$ the cardinality of the dataset, $d$ the dimensionality.

{\bf MILLIONSONGS \cite{BertinMahieux2011TheMS}} ($n=\num[group-separator={,}]{463715}$, $d=90$, regression).
%
We use the same preprocessing, kernel and $\sigma$ as \cite{conf/colt/ZhangDW13}.
In Table~\ref{MS_table} we observe our result when we choose \num[group-separator={,}]{10000} Nystrom centers
and $lambda = 10^{-6}$.
Increasing the centers to \num[group-separator={,}]{50000} we get a MSE of $79.20$ and a Relative error of $4.49\times10^{-3}$ in $630$ \textit{sec}.

\begin{table}[h]
  \caption{MILLIONSONGS and SUSY Datasets. $\dagger = $ time obtained by \cite{Alves2016StackingML} working on a single machine.}
  \label{MS_table}
  \centering
    \begin{tabular}{lccc}
      \toprule
      & \multicolumn{3}{c}{MILLIONSONGS Dataset} \\
      \cmidrule{2-4}
    %   \textbf{MILLIONSONGS}
           & MSE   &Relative Error            & Time(\textit{sec})\\
      \midrule
      Falcon                      & \textbf{80.30}  &$\mathbf{4.51\times10^{-3}}$    & \textbf{55}  \\
      Prec. KRR\cite{avron2016faster}                 &-               &$4.58\times10^{-3}$    &289 \\
      Hierarchical \cite{Chen2016HierarchicallyCK}                 &-               &$4.56\times10^{-3}$    &293 \\
      D\&C \cite{conf/colt/ZhangDW13}            & 80.35    &-             & 737 \\
      Rand. Feat. \cite{conf/colt/ZhangDW13}     & 80.93    &-            & 772 \\
      Nystrom \cite{conf/colt/ZhangDW13}             & 80.38    &-            & 876 \\
      ADMM\cite{avron2016faster}                 &-               &$5.01\times10^{-3}$    &958 \\
    %   \bottomrule
    %   \toprule
    \midrule
      & \multicolumn{3}{c}{SUSY Dataset} \\
      \cmidrule{2-4}
    \textbf{SUSY}
                                 & Class error    & AUC    & Time (\textit{min})   \\
      \midrule
      Falcon                          & \textbf{19.4\%}  &0.877   & \textbf{4} \\
      EigenPro \cite{ma2017diving}    & 19.8\%         &-       & 6 \\
      Hierarchical \cite{Chen2016HierarchicallyCK}                   & 20.1\%         &-       & 40 \\
      BDT \cite{baldi2014searching}                     &-              & 0.863     &- \\
      NN \cite{baldi2014searching}                   &-                 & 0.875    & -\\
      DNN \cite{baldi2014searching}                  &-                  &\textbf{0.879}     & $4680^\dagger$  \\
      \bottomrule
    \end{tabular}
\end{table}

{\bf TIMIT}~($n = \num[group-separator={,}]{1124823}$, $d = 440$, multiclass classification).
%
In this experiment we used the same preprocessed dataset of [Mikhal].
In the results of Table~\ref{YHT_table} Falcon exploits a Gaussian Kernel of width $\sigma = 15$,
$\lambda = 10^{-9}$ and $10^5$ Nystrom centers.
% The results in Table~\ref{TIMIT_table}, shows that Falcon outperform most of the competitors
% (including a DNN and full KRR) in a small amount of time and only one machine. (IBM?)
% Notice that in respect to most competitors we train only on half the number of points. (WHY)
% **Our dataset adopts 10ms frames and drops the glottal stop \'q\' related labels,
% thus we ignore the relevant frames in core test set (1.2\% of total test set).
% Note that in the worst case, if we mislabel all these frames, the corresponding
% frame-level classification error will drop from 32.6\% to 33.39\%.**

% \begin{table}[h]
%   \caption{TIMIT Dataset. $\ddagger = $ time obtained on a cluster of 128 Amazon r3.2xlarge machines.}
%   \label{TIMIT_table}
%   \centering
%
%   \begin{tabular}{lcccccc}
%     \toprule
%     TIMIT                         & Class error   & Time (\textit{hours})   \\
%     \midrule
%     Falcon                      & 32.3\% & \textbf{1.5} \\
%     BCD Rand. Feat. \cite{tu2016large}   & 34.0\% & $1.7^\ddagger$ \\
%     BCD Nystrom \cite{tu2016large}           & 33.7\% & $1.7^\ddagger$ \\
%     EigenPro \cite{ma2017diving}            & 32.6\% & 3.9 \\
%     KRR \cite{tu2016large}                   & 33.5\% & $8.3^\ddagger$ \\
%     DNN \cite{May2017KernelAM}                   & 32.4\% & -   \\
%     ????Kernels \cite{May2017KernelAM}    & \textbf{30.9\%} & -   \\
%     Ensemble \cite{Huang2014KernelMM}          & 33.5\% & -   \\
%     \bottomrule
%   \end{tabular}
% \end{table}



{\bf SUSY}~($n = 5\times10^6$, $d = 18$, binary classification).
%
Results for Falcon with a Gaussina kernel of width $\sigma = 5$, $\lambda = 10^{-6}$ and $10^4$ Nystrom centers are shown
in Table~\ref{MS_table}.

% \begin{table}[h]
%     \caption{SUSY Dataset. $\dagger = $ time obtained by \cite{Alves2016StackingML} working on a single machine.}
%     \label{SUSY_table}
%     \centering
%
%     \begin{tabular}{lccc}
%         \toprule
%         SUSY                           & Class error    & AUC    & Time (\textit{min})   \\
%         \midrule
%         Falcon                          & \textbf{19.4\%}  &0.877   & \textbf{4} \\
%         EigenPro \cite{ma2017diving}    & 19.8\%         &-       & 6 \\
%         Hierarchical \cite{Chen2016HierarchicallyCK}                   & 20.1\%         &-       & 40 \\
%         BDT \cite{baldi2014searching}                     &-              & 0.863     &- \\
%         NN \cite{baldi2014searching}                   &-                 & 0.875    & -\\
%         DNN \cite{baldi2014searching}                  &-                  &\textbf{0.879}     & $4680^\dagger$  \\
%         \bottomrule
%     \end{tabular}
% \end{table}

\begin{table}[h]
    \caption{YELP, HIGGS and TIMIT Datasets. $\dagger = $ time obtained by \cite{Alves2016StackingML} working on a single machine. $\ddagger = $ time obtained on a cluster of 128 Amazon r3.2xlarge machines.}
    \label{YHT_table}
    \begin{subtable}[]{0.3\linewidth}
        \centering
    \begin{tabular}{lcc}
        \toprule
        & \multicolumn{2}{c}{YELP Dataset} \\
        \cmidrule{2-3}
        % \textbf{YELP}
                                               & RMSE              & Time (\textit{mins}) \\
        \midrule
        Falcon                      & \textbf{0.833}    & $\textbf{20}$ \\
        BCD Hashing \cite{tu2016large}                       & 0.949             & $42^\ddagger$ \\
        BCD Nystrom \cite{tu2016large}                       & 0.861             & $60^\ddagger$ \\
        KRR  \cite{tu2016large}           & 0.854             & $500^\ddagger$ \\
        % \bottomrule
        % \toprule
         \midrule
         & \multicolumn{2}{c}{HIGGS Dataset} \\
         \cmidrule{2-3}
        %  \textbf{HIGGS}
                                    & AUC   & Time (\textit{hours})   \\
         \midrule
         Falcon                      & 0.818 & \textbf{3} \\
         BDT \cite{baldi2014searching}                 & 0.810 & - \\
         NN \cite{baldi2014searching}                  & 0.816 & - \\
         DNN \cite{baldi2014searching}                 & \textbf{0.885} & $78^\dagger$ \\
        \bottomrule
    \end{tabular}
\end{subtable}
\hspace{2.2cm}
\begin{subtable}[]{0.3\linewidth}
        \centering
    \begin{tabular}{lcc}
      \toprule
      & \multicolumn{2}{c}{TIMIT Dataset} \\
      \cmidrule{2-3}
    % \textbf{TIMIT}
                               & Class error   & Time (\textit{hours})   \\
      \midrule
      Falcon                      & 32.3\% & \textbf{1.5} \\
      BCD Rand. Feat. \cite{tu2016large}   & 34.0\% & $1.7^\ddagger$ \\
      BCD Nystrom \cite{tu2016large}           & 33.7\% & $1.7^\ddagger$ \\
      EigenPro \cite{ma2017diving}            & 32.6\% & 3.9 \\
      KRR \cite{tu2016large}                   & 33.5\% & $8.3^\ddagger$ \\
      DNN \cite{May2017KernelAM}                   & 32.4\% & -   \\
      ????Kernels \cite{May2017KernelAM}    & \textbf{30.9\%} & -   \\
      Ensemble \cite{Huang2014KernelMM}          & 33.5\% & -   \\
      \bottomrule
    \end{tabular}
    \end{subtable}
\end{table}

{\bf YELP}~~($n = 1.5 \times 10^6$, $d = 6.52 \times 10^7$, regression).
%
We test Falcon on the same dataset used by \cite{tu2016large},
For preprocessing we extract the 3-grams from the plain text with the same pipeline as \cite{tu2016large},
then we map them in a sparse vector which records if the 3-gram is present or not in the example.
For the results presented in Table~\ref{YHT_table} Falcon uses a linear kernel with $5\times10^4$ Nystorm centers.
Increasing the number of centers to $10^5$ we get a RMSE of $0.8280$ in $50$ minutes.

% \begin{table}[h]
%     \caption{YELP Dataset. $\ddagger = $ time obtained on a cluster of 128 Amazon r3.2xlarge machines.}
%     \label{YELP_table}
%     \begin{subtable}[t]{.45\linewidth}
%     \centering
%     \begin{tabular}{lcc}
%         \toprule
%         YELP                                       & RMSE              & Time (\textit{mins}) \\
%         \midrule
%         Falcon                      & \textbf{0.833}    & $\textbf{20}$ \\
%         BCD Hashing \cite{tu2016large}                       & 0.949             & $42^\ddagger$ \\
%         BCD Nystrom \cite{tu2016large}                       & 0.861             & $60^\ddagger$ \\
%         KRR  \cite{tu2016large}           & 0.854             & $500^\ddagger$ \\
%         \bottomrule
%     \end{tabular}
% \end{subtable}\hfill
%     \begin{subtable}[t]{.45\linewidth}
%         \begin{tabular}{lcc}
%         \toprule
%         HIGGS                           & AUC   & Time (\textit{hours})   \\
%         \midrule
%         Falcon                      & 0.818 & \textbf{3} \\
%         BDT \cite{baldi2014searching}                 & 0.810 & - \\
%         NN \cite{baldi2014searching}                  & 0.816 & - \\
%         DNN \cite{baldi2014searching}                 & \textbf{0.885} & $78^\dagger$ \\
%         \bottomrule
%         \end{tabular}
%     \end{subtable}
% \end{table}

{\bf HIGGS}~($n = 1.1\times 10^6$, $d = 28$, binary classification).
%
Results from Table~\ref{YHT_table} are obtained using a Gaussian Kernel of width $\sigma = 5$, $\lambda = 1\times10^{-8}$ and
$1\times10^5$ Nystrom centers.
If we enrich our model a bit using a Gaussian kernel with diagona matrix width learned with cross validation,
Falcon reaches an AUC of $0.830$.


% \begin{table}[h]
%     \caption{HIGGS Dataset. $\dagger = $ time obtained by \cite{Alves2016StackingML} working on a single machine.}
%     \label{HIGGS_table}
%     \centering
%     \begin{tabular}{lcc}
%         \toprule
%         HIGGS                         & AUC   & Time (\textit{hours})   \\
%         \midrule
%         Falcon                      & 0.818 & \textbf{3} \\
%         BDT \cite{baldi2014searching}                 & 0.810 & - \\
%         NN \cite{baldi2014searching}                  & 0.816 & - \\
%         DNN \cite{baldi2014searching}                 & \textbf{0.885} & $78^\dagger$ \\
%         \bottomrule
%         \toprule
%         YELP                                       & RMSE              & Time (\textit{mins}) \\
%         \midrule
%         Falcon                      & \textbf{0.833}    & $\textbf{20}$ \\
%         BCD Hashing \cite{tu2016large}                       & 0.949             & $42^\ddagger$ \\
%         BCD Nystrom \cite{tu2016large}                       & 0.861             & $60^\ddagger$ \\
%         KRR  \cite{tu2016large}           & 0.854             & $500^\ddagger$ \\
%         \bottomrule
%     \end{tabular}
% \end{table}

